Evaluating Pre-Trained Models for User Feedback Analysis in Software Engineering: A Study on Classification of App-Reviews

Context: Mobile app reviews written by users on app stores or social media are significant resources for app developers.Analyzing app reviews have proved to be useful for many areas of software engineering (e.g., requirement engineering, testing). Automatic classification of app reviews requires extensive efforts to manually curate a labeled dataset. When the classification purpose changes (e.g. identifying bugs versus usability issues or sentiment), new datasets should be labeled, which prevents the extensibility of the developed models for new desired classes/tasks in practice. Recent pre-trained neural language models (PTM) are trained on large corpora in an unsupervised manner and have found success in solving similar Natural Language Processing problems. However, the applicability of PTMs is not explored for app review classification Objective: We investigate the benefits of PTMs for app review classification compared to the existing models, as well as the transferability of PTMs in multiple settings. Method: We empirically study the accuracy and time efficiency of PTMs compared to prior approaches using six datasets from literature. In addition, we investigate the performance of the PTMs trained on app reviews (i.e. domain-specific PTMs) . We set up different studies to evaluate PTMs in multiple settings: binary vs. multi-class classification, zero-shot classification (when new labels are introduced to the model), multi-task setting, and classification of reviews from different resources. The datasets are manually labeled app review datasets from Google Play Store, Apple App Store, and Twitter data. In all cases, Micro and Macro Precision, Recall, and F1-scores will be used and we will report the time required for training and prediction with the models.

==> Discussions.tex <==
include D7: One point of discussion could be the ptms ability for highly imbalanced dataset



\textcolor{red}{Add the Kaggle data to the changes, additional to the MSR RR. }
\textcolor{black}{To have a comparison, we also test the Prior Approaches for this setting. From the {Prior} approaches, {AR-Miner} does not require training. For the other approaches, we train them on the App Store reviews of \textit{Dataset 2} and test them on Tweets in \textit{Dataset 2}. We only apply this setting for these approaches, as we already know they are developed for classification of app reviews not for Twitter. So, we do not train them on Twitter data and test them on app reviews.}



==> discussions.tex <==
\section{Discussions and Implications}
\label{sec:disc}

% We should refer to the motivations of this study to elaborate on these. for example, developers can use the PTMs and apply them directly on their custom classification task, without worries about labeling new data for new classes. }

%In this section, we discuss the lesson learned from from our study and how the findings can be helpful for the researchers, practitioners, and app developers or companies.
Implications for users\footnote{Here, the users can be developers, practitioners, or researchers who want to use the studied models to classify issues related to mobile apps from user feedbacks.} 

\textbf{Prior Approaches: Deep learning with word embedding can be used for app issue classification when one does not want to use PTMs.} From the prior approaches, Deep Learning Technique leveraging Word Embedding (DL+WE) generated the best results for predicting the correct classes of app reviews (RQ1), followed closely by the Ensemble Method. DL+WE also took the least amount of time to predict the classes, whereas SUR-Miner took the second least amount of time. However, if no labels are available to train the mentioned models, AR-Miner should be used, which utilizes topic modeling to separate the classes of app reviews.

\textbf{Prior Approaches vs. PTMs: If the prediction time does not matter much but high performance is required, PTMs should be used to classify app issues.}
From the results of RQ1, we observed that all PTMs outperformed the prior approaches (except for 1 out of 28 cases) to predict classes accurately. RoBERTa and ALBERT scored the highest F1-scores in most of the datasets among D1 to D7. Compared with the fastest prior approach, ALBERT has the lowest, and XLNET has the highest increase in prediction time. 
Consequently, it is worth applying PTMs for app-review classification if the developer, researcher, or software engineer can spare marginally additional time to achieve higher prediction scores.


{\textbf{Training Custom PTMs.}}
The inclusion of app reviews in the pre-training corpus allows PTMs to classify user feedbacks with higher F1 scores. 
We have pre-trained three models of both ALBERT and RoBERTa with three different sizes of corpora. 
%The BASE, MEDIUM, and LARGE iterations of both ALBERT and RoBERTa incorporate 2.8M, 5.6M, and 10M app reviews to the initial pre-training corpus, respectively.
This experiment found that more domain-specific information during the pre-training helps the newly trained PTMs yield better predictions of app reviews. C-ALBERT and C-RoBERTa models can improve the ALBERT and RoBERTa scores for up to $\sim$13\% and $\sim$14\%, respectively. %-BASE, MEDIUM, and LARGE yield $\sim$[0.8-9\%], $\sim$[1-10\%], and $\sim$[4-13\%] increase in performance, respectively; whereas, RoBERTa-BASE, MEDIUM, and LARGE yield $\sim$[1-8\%], $\sim$[3-10\%], and $\sim$[5-14\%] increase in performance, respectively. 
\textcolor{red}{In all Custom PTMs, there is a lack of significant variance with regard to the prediction time reported for those that do not include app reviews into the pretraining corpus as the prediction time depends solely on the prediction stage rather than the training step.
}


\textbf{Binary vs. Multi-class.}
All PTMs and Prior approaches performed better in binary classification than in multiclass classification.
From Tables \ref{table:RQ3_binary_a} and \ref{table:RQ3_binary_b} , we observe that converting or trimming a multi-class dataset to a binary class dataset help all the prior and PTM approaches to yield better performance. Prior approaches are improved by 0 to $\sim$3\%, whereas the gain for the PTMs ranges from 1 to $\sim$7\%. For binary classification, all PTM approaches performed better than they did for multi-class classifications, and the performance boost produced by readily-available PTMs is proportionate to the performance boost produced by custom PTMs.

\textbf{Zero-shot.}
All PTMs can be implemented in a Zero-Shot setting and yield adequate performance.
The only Prior approach that can be used directly in this setting is AR-Miner which is based on topic modeling. 
All the readily available and custom PTMs are fine-tuned on NLI dataset for Inference classification task. Due to the fact that these PTM models had not been exposed to any instances of the datasets in our study in the zero-shot setting, they are expected to perform worse than their reported performance in Tables \ref{table:RQ1_ptm}, \ref{table:RQ2_cptm_albert}, and \ref{table:RQ2_cptm_roberta}. 
%Except for one case of \textit{$D_5$} where \textit{PTM-ALBERT-NLI} performed worse than AR-MINER, PTMs beat AR-Miner by a large margin in all datasets. Among the PTMs, \textit{RoBERTa-LARGE-NLI} yielded the best F1-scores in all the datasets. 
The Custom-PTMs pre-trained with domain-specific knowledge could not outperform the readily available \textit{RoBERTa-LARGE-MNLI}. This can be related to the dataset used for its training, which is a much larger dataset than the NLI datasets we used to train our PTMs.  
Although the CPTMs cannot beat the \textit{RoBERTa-LARGE-MNLI} model, it is notable that these CPTMs are smaller models and the \textit{RoBERTa-LARGE-MNLI} model is a very large language model; but still, the CPTMs we studied achieve significant improvements compared to their general domain PTMs in this setting. 


\textbf{Custom PTMs vs. PTMs.}
Customized PTMs that are pre-trained with the app review data have the best performance in all settings: binary classification, multi-class classification, multi-task, and multi-resource setting. Even for zero shot setting, they perform better than all the other models (except for RoBERTa-LARGE-MNLI that is trained on a much larger NLI data). 
The benefit of using custom PTMs, specifically RoBERTa-based ones, compared to PTMs, is more obvious for the multi-task and multi-resource setting in RQ3-3 and RQ3-4. 
Interestingly, the PTMs do not perform well in the multi-task and multi-resource setting, while CPTMs have the highest scores. The PTMs in these two settings perform lower than the Ensemble and DL+WE models. But, the best CPTMs achieve scores of above 90\% for multi-task and 86\% and 92\% F1 score for multi-resource. 
Other than achieving the best score, CPTMs have the lowest prediction time among all models for multi-class classification, multi-task, and multi-resource settings.
They also achieve the lowest prediction time for some of the datasets in binary classification.
Our results for RQ3-4 confirms that using over the shelf PTMs might not be the best option when classifying issues for app reviews in all settings.
PTMs can still have good performance in binary and multi-class classification. But for harder scenarios (i.e., zero shot, multi-task, and multi-resource), pre-training them with domain specific data increases their performance and reduces their prediction time. 
Moreover, the more app review data is used in the pre-training of CPTMs, the better their performence is.



\textbf{PTMs vs. Prior Approaches.}
For the multi-class classification (RQ1), PTMs perform significantly better than the Prior Approaches for most datasets. For Dataset $D_2$, the difference in the scores among the two groups is not much, but when we consider $D_7$, the results of PTMs are almost 10 F1 score higher than the best Prior Approach. The prediction times also vary, but, some PTMs can predict the labels with approximately the same time as the best Prior Approaches (Ensemble and DL+WE). 
For binary classification, the best Prior Approaches achieve scores of below 90\% and mostly in the low 80\% F1 score. But, the F1 scores of PTMs are mainly above 90\% and the Custom PTMs have even higher scores. 
However, for multi-resource setting (RQ3-4), the Ensemble and DL+WE have better F1 scores than all PTMs, but not higher than CPTMs. This result is interesting, showing that the learned knowledge about the app review domain for issue classification is important in this setting, no matter if the model is trained on App Store data and tested on Twitter data, or vice versa. This is confirmed by the obtained results of the C-RoBERTa-LARGE, which have the highest scores among all models in this setting. 

%\subsection{\textbf{Both PTMs and Prior approaches yield promising results while classifying of app reviews collected from multiple resources}}

%The dataset \textit{$D_2$} contains labeled app reviews from two different sources: the App Store and Twitter. In the multi-resource setting, we have fine-tuned all PTM approaches on app reviews from App Store, and we have tested them on app reviews collected using another resource, i.e., Twitter. Being a topic modeling approach, \textit{AR-Miner} is again the only eligible prior approach to be considered in this setting.
%From all the available approaches, SUR-Miner, Ensemble, and DL+WE had shown an increase in their performance by ($\sim$2\% to $\sim$5\%). For readily available PTMs, we observe significant performance reduction ($\sim$13\% to $\sim$31\%) for micro F1-scores. In this setting, Custom-PTMs produced micro-F1 scores with comparatively less performance reduction. Among the CPTM-ALBERTs, the \textit{CPTM-ALBERT-LARGE} model produced the best, and \textit{CPTM-ALBERT-BASE} model produced the least micro F1-score. In the CPTM-RoBERTa group, the corresponding performance reduction was even smaller than in CPTM-ALBERTs.

{\textbf{The Performance of Models.}}
\textcolor{black}{Readily available PTMs are generally outperforming the Prior approaches as these Prior approaches need to learn about both Natural language and classification tasks from the training set, whereas PTMs can put more focus on learning about the classification tasks from the training set as PTMs already have extensive knowledge on Natural Languages from pre-training.}

\textcolor{black}{On the other hand, custom PTMs, pre-trained on domain specific data along with general domain data, generally perform better than readily available PTMs as the custom PTMs acquire more syntactic and semantic knowledge about the domain during their pre-training. As app reviews have some unique attributes (e.g., shortness of texts, excessive use of stop-words, noise), the domain specific knowledge helps the custom PTMs to better classify the texts related to the domain they are trained on.}

%\textcolor{blue}{We have observed that the Prior approaches can match or beat PTMs for multi-task learning. We conjecture that Prior approaches' knowledge about the App Store app review domain appeared to be an advantage for them, whereas PTMs with a broader knowledge of the natural language do not benefit in this setting, unless the domain knowledge is incorporated in their pre-training.}

\textcolor{blue}{For the multi-resource classification, we noticed that in the second part of the setting, where we have trained/ fine-tuned the models on tweets and tested them on app reviews, all the PTMs performed relatively better and LARGE models (both C-ALBERT and C-RoBERTa) reported a smaller decrease in performance, as opposed to the first part where we have fine-tuned the models on app reviews and tested them on tweets. In both parts of the multi-resource setting, Prior approaches (Ensemble and DL+WE) performed better than counterparts in other settings. 
%We conjecture that Prior approaches' knowledge about the app review domain appeared to be an advantage for them, whereas PTMs with a broader knowledge of the natural language do not benefit in this setting, unless the domain knowledge is incorporated in their pre-training.
We can attribute these findings to the ratio of training and testing sets. In the first part of this setting, models were trained/ fine-tuned on the app reviews of the dataset $D_2$, which have a higher number of labeled tweets (10,364) than the app reviews (6,406). This higher volume of data in the training set helped the PTMs and Prior approaches yield smaller performance reductions and achieve higher performance in the second part of multi-resource, in terms of F1-score. }

\subsection{\textbf{Implications}}
\textcolor{red}{From our study, we suggest to use Pre-trained models for app review classification tasks as for the same amount of training data, PTMs have found to be performing better than the Prior approaches. Among all the PTMs we have incorporated in our study, ALBERT and RoBERTa have outperformed other PTMs and prior approaches. From the performance yielded by custom PTMs, we can suggest if developers or researchers have an abundance of unlabeled domain-specific data, they should consider simultaneous pre-training for their selected PTMs to obtain higher prediction accuracy.}

\textcolor{red}{As a design recommendation for modeling the classification problem, we suggest designing it as balanced binary rather than as multi-class imbalanced since all approaches perform well on the former task. PTMs have proved effective in all four settings of our last research question, so we recommend practitioners adopt them for all app review classification tasks.}
